Online Local Boosting: improving performance in online decision trees

As more data are produced each day, and faster, data stream mining is growing in importance, making clear the need for algorithms able to fast process these data. Data stream mining algorithms are meant to be solutions to extract knowledge online, specially tailored from continuous data problem. Many of the current algorithms for data stream mining have high processing and memory costs. Often, the higher the predictive performance, the higher these costs. To increase predictive performance without largely increasing memory and time costs, this paper introduces a novel algorithm, named Online Local Boosting (OLBoost), which can be combined into online decision tree algorithms to improve their predictive performance without modifying the structure of the induced decision trees. For such, OLBoost applies a boosting to small separate regions of the instances space. Experimental results presented in this paper show that by using OLBoost the online learning decision tree algorithms can significantly improve their predictive performance. Additionally, it can make smaller trees perform as good or better than larger trees.

==> ESANN_OLBoost_ACC.tex <==
% %\begin{figure}[!htbp] \centering 
% \scalebox{1.0}{
% \begin{tikzpicture}[xscale=1]
% \node (Label) at  (00.8167,0.7) {\scriptsize{CD = 0.45}}; % the label
% \draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, thick, color = black](00.6667, 0.5) -- (00.9667, 0.5);
% \foreach \x in {00.6667,00.9667} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);

% \draw[gray, thick](00.6667, 0) -- (04.0000, 0);
% \foreach \x in {00.6667,01.3333,02.0000,02.6667,03.3333,04.0000}\draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
% \node (Label) at (00.6667,0.2) {\scriptsize{1}};
% \node (Label) at (01.3333,0.2) {\scriptsize{2}};
% \node (Label) at (02.0000,0.2) {\scriptsize{3}};
% \node (Label) at (02.6667,0.2) {\scriptsize{4}};
% \node (Label) at (03.3333,0.2) {\scriptsize{5}};
% \node (Label) at (04.0000,0.2) {\scriptsize{6}};
% \draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, thick, color = black](02.1167,-00.2500) -- ( 02.5033,-00.2500);
% \node (Point) at (01.1733, 0){};  \node (Label) at (-0.4,-00.3000){\scriptsize{OLBoost\_VFDT}}; \draw (Point) |- (Label);
% \node (Point) at (01.7133, 0){};  \node (Label) at (-0.4,-00.6000){\scriptsize{OLBoost\_SVFDT-II}}; \draw (Point) |- (Label);
% \node (Point) at (02.1667, 0){};  \node (Label) at (-0.4,-00.9000){\scriptsize{OLBoost\_SVFDT-I}}; \draw (Point) |- (Label);
% \node (Point) at (03.4867, 0){};  \node (Label) at (5.5,-00.3000){\scriptsize{SVFDT-I}}; \draw (Point) |- (Label);
% \node (Point) at (02.9867, 0){};  \node (Label) at (5.5,-00.6000){\scriptsize{SVFDT-II}}; \draw (Point) |- (Label);
% \node (Point) at (02.4533, 0){};  \node (Label) at (5.5,-00.90 00){\scriptsize{VFDT}}; \draw (Point) |- (Label);
% \end{tikzpicture}
% }
% %\vspace{-10pt}
% %\caption{Critical distance diagram for Nemenyi test with accuracy results.}
% \label{fig:nemenyi_acc}
% %\end{figure}

%\begin{figure}
%\centering
\scalebox{1.0}{
\begin{tikzpicture}[xscale=1]
\node (Label) at (2.1367567501848885, 0.7){\tiny{CD = 2.27}}; % the label
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black] (1.0,0.5) -- (3.273513500369777,0.5);
\foreach \x in {1.0, 3.273513500369777} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);

\draw[gray, thick](1.0,0) -- (6.0,0);
\foreach \x in {1.0,2.0,3.0,4.0,5.0,6.0} \draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
\node (Label) at (1.0,0.2){\tiny{1}};
\node (Label) at (2.0,0.2){\tiny{2}};
\node (Label) at (3.0,0.2){\tiny{3}};
\node (Label) at (4.0,0.2){\tiny{4}};
\node (Label) at (5.0,0.2){\tiny{5}};
\node (Label) at (6.0,0.2){\tiny{6}};
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](1.5863636363636364,-0.25) -- (3.4136363636363636,-0.25);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](3.0409090909090915,-0.4) -- (5.095454545454546,-0.4);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](4.995454545454546,-0.25) -- (5.731818181818182,-0.25);
\node (Point) at (1.6363636363636365, 0){};\node (Label) at (0.5,-0.8500000000000001){\scriptsize{OLBoost\_VFDT}}; \draw (Point) |- (Label);
\node (Point) at (2.1818181818181817, 0){};\node (Label) at (0.5,-1.1500000000000001){\scriptsize{OLBoost\_SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (3.0909090909090913, 0){};\node (Label) at (0.5,-1.4500000000000002){\scriptsize{OLBoost\_SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (5.6818181818181825, 0){};\node (Label) at (6.5,-0.8500000000000001){\scriptsize{SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (5.045454545454546, 0){};\node (Label) at (6.5,-1.1500000000000001){\scriptsize{SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (3.3636363636363638, 0){};\node (Label) at (6.5,-1.4500000000000002){\scriptsize{VFDT}}; \draw (Point) |- (Label);
\end{tikzpicture}
}
%\caption{Nemenyi - parsed acc mean.csv}
\label{fig:nemenyi_acc}
%\end{figure}


==> ESANN_OLBoost_MEM.tex <==
% %\begin{figure}[!htbp] \centering
% \scalebox{1.0}{
% \begin{tikzpicture}[xscale=1.0]
% \node (Label) at  (00.8167,0.7) {\scriptsize{CD = 0.45}}; % the label
% \draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, thick, color = black](00.6667, 0.5) -- (00.9667, 0.5);
% \foreach \x in {00.6667,00.9667} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);

% \draw[gray, thick](00.6667, 0) -- (04.0000, 0);
% \foreach \x in {00.6667,01.3333,02.0000,02.6667,03.3333,04.0000}\draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
% \node (Label) at (00.6667,0.2) {\scriptsize{1}};
% \node (Label) at (01.3333,0.2) {\scriptsize{2}};
% \node (Label) at (02.0000,0.2) {\scriptsize{3}};
% \node (Label) at (02.6667,0.2) {\scriptsize{4}};
% \node (Label) at (03.3333,0.2) {\scriptsize{5}};
% \node (Label) at (04.0000,0.2) {\scriptsize{6}};
% \draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, thick, color = black](01.6367,-00.2500) -- ( 01.9900,-00.2500);
% \node (Point) at (0.7400, 0){};  \node (Label) at (-0.4,-00.3000){\footnotesize{SVFDT-I}}; \draw (Point) |- (Label);
% \node (Point) at (01.6867, 0){};  \node (Label) at (-0.4,-00.6000){\footnotesize{SVFDT-II}}; \draw (Point) |- (Label);
% \node (Point) at (01.9400, 0){};  \node (Label) at (-0.4,-00.9000){\footnotesize{OLBoost\_SVFDT-I}}; \draw (Point) |- (Label);
% \node (Point) at (03.8933, 0){};  \node (Label) at (5.5,-00.3000){\footnotesize{OLBoost\_VFDT}}; \draw (Point) |- (Label);
% \node (Point) at (03.0267, 0){};  \node (Label) at (5.5,-00.6000){\footnotesize{OLBoost\_SVFDT-II}}; \draw (Point) |- (Label);
% \node (Point) at (02.6933, 0){};  \node (Label) at (5.5,-00.9000){\footnotesize{VFDT}}; \draw (Point) |- (Label);
% \end{tikzpicture}
% }
% %\vspace{-10pt}
% %\caption{Critical distance diagram for Nemenyi test with memory consumption}
% \label{fig:nemenyi_mem}
% %\end{figure}

%\begin{figure}
%\centering
\scalebox{1.0}{
\begin{tikzpicture}[xscale=1]
\node (Label) at (2.1367567501848885, 0.7){\tiny{CD = 2.27}}; % the label
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black] (1.0,0.5) -- (3.273513500369777,0.5);
\foreach \x in {1.0, 3.273513500369777} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);

\draw[gray, thick](1.0,0) -- (6.0,0);
\foreach \x in {1.0,2.0,3.0,4.0,5.0,6.0} \draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
\node (Label) at (1.0,0.2){\tiny{1}};
\node (Label) at (2.0,0.2){\tiny{2}};
\node (Label) at (3.0,0.2){\tiny{3}};
\node (Label) at (4.0,0.2){\tiny{4}};
\node (Label) at (5.0,0.2){\tiny{5}};
\node (Label) at (6.0,0.2){\tiny{6}};
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](0.9954545454545454,-0.25) -- (3.0954545454545452,-0.25);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](2.2681818181818185,-0.4) -- (4.459090909090909,-0.4);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](4.131818181818182,-0.25) -- (6.05,-0.25);
\node (Point) at (1.0454545454545454, 0){};\node (Label) at (0.5,-0.8500000000000001){\scriptsize{SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (2.3181818181818183, 0){};\node (Label) at (0.5,-1.1500000000000001){\scriptsize{SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (3.0454545454545454, 0){};\node (Label) at (0.5,-1.4500000000000002){\scriptsize{OLBoost\_SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (6.0, 0){};\node (Label) at (6.5,-0.8500000000000001){\scriptsize{OLBoost\_VFDT}}; \draw (Point) |- (Label);
\node (Point) at (4.409090909090909, 0){};\node (Label) at (6.5,-1.1500000000000001){\scriptsize{OLBoost\_SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (4.181818181818182, 0){};\node (Label) at (6.5,-1.4500000000000002){\scriptsize{VFDT}}; \draw (Point) |- (Label);
\end{tikzpicture}
}
%\caption{Nemenyi - parsed memory size.csv}
\label{fig:nemenyi_mem}
%\end{figure}


==> ESANN_OLBoost_TIME.tex <==
% %\begin{figure}[!htbp] \centering
% \scalebox{1.0}{
% \begin{tikzpicture}[xscale=1.0]
% \node (Label) at  (00.8167,0.7) {\scriptsize{CD = 0.45}}; % the label
% \draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, thick, color = black](00.6667, 0.5) -- (00.9667, 0.5);
% \foreach \x in {00.6667,00.9667} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);

% \draw[gray, thick](00.6667, 0) -- (04.0000, 0);
% \foreach \x in {00.6667,01.3333,02.0000,02.6667,03.3333,04.0000}\draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
% \node (Label) at (00.6667,0.2) {\scriptsize{1}};
% \node (Label) at (01.3333,0.2) {\scriptsize{2}};
% \node (Label) at (02.0000,0.2) {\scriptsize{3}};
% \node (Label) at (02.6667,0.2) {\scriptsize{4}};
% \node (Label) at (03.3333,0.2) {\scriptsize{5}};
% \node (Label) at (04.0000,0.2) {\scriptsize{6}};
% \draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, thick, color = black](01.2567,-00.2500) -- ( 01.4967,-00.2500);
% \draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, thick, color = black](03.0500,-00.2500) -- ( 03.4433,-00.2500);
% \node (Point) at (01.3067, 0){};  \node (Label) at (-0.4,-00.3000){\footnotesize{SVFDT-I}}; \draw (Point) |- (Label);
% \node (Point) at (01.4333, 0){};  \node (Label) at (-0.4,-00.6000){\footnotesize{VFDT}}; \draw (Point) |- (Label);
% \node (Point) at (01.4467, 0){};  \node (Label) at (-0.4,-00.9000){\footnotesize{SVFDT-II}}; \draw (Point) |- (Label);
% \node (Point) at (03.3933, 0){};  \node (Label) at (5.5,-00.3000){\footnotesize{OLBoost\_SVFDT-II}}; \draw (Point) |- (Label);
% \node (Point) at (03.3000, 0){};  \node (Label) at (5.5,-00.6000){\footnotesize{OLBoost\_VFDT}}; \draw (Point) |- (Label);
% \node (Point) at (03.1000, 0){};  \node (Label) at (5.5,-00.9000){\footnotesize{OLBoost\_SVFDT-I}}; \draw (Point) |- (Label);
% \end{tikzpicture}
% }
% %\vspace{-10pt}
% %\caption{Critical distance diagram for Nemenyi test with time results.}
% \label{fig:nemenyi_time}
% %\end{figure}

%\begin{figure}
%\centering
\scalebox{1.0}{
\begin{tikzpicture}[xscale=1]
\node (Label) at (2.1367567501848885, 0.7){\tiny{CD = 2.27}}; % the label
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black] (1.0,0.5) -- (3.273513500369777,0.5);
\foreach \x in {1.0, 3.273513500369777} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);

\draw[gray, thick](1.0,0) -- (6.0,0);
\foreach \x in {1.0,2.0,3.0,4.0,5.0,6.0} \draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
\node (Label) at (1.0,0.2){\tiny{1}};
\node (Label) at (2.0,0.2){\tiny{2}};
\node (Label) at (3.0,0.2){\tiny{3}};
\node (Label) at (4.0,0.2){\tiny{4}};
\node (Label) at (5.0,0.2){\tiny{5}};
\node (Label) at (6.0,0.2){\tiny{6}};
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](1.768181818181818,-0.25) -- (2.3227272727272728,-0.25);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](4.677272727272728,-0.25) -- (5.140909090909091,-0.25);
\node (Point) at (1.8181818181818181, 0){};\node (Label) at (0.5,-0.65){\scriptsize{SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (2.0, 0){};\node (Label) at (0.5,-0.95){\scriptsize{VFDT}}; \draw (Point) |- (Label);
\node (Point) at (2.272727272727273, 0){};\node (Label) at (0.5,-1.25){\scriptsize{SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (5.090909090909091, 0){};\node (Label) at (6.5,-0.65){\scriptsize{OLBoost\_VFDT}}; \draw (Point) |- (Label);
\node (Point) at (5.090909090909091, 0){};\node (Label) at (6.5,-0.95){\scriptsize{OLBoost\_SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (4.7272727272727275, 0){};\node (Label) at (6.5,-1.25){\scriptsize{OLBoost\_SVFDT-I}}; \draw (Point) |- (Label);
\end{tikzpicture}
}
%\caption{Nemenyi - parsed time(s).csv}
\label{fig:nemenyi_time}
%\end{figure}


==> old/ESANN_OLBoost_ACC.tex <==
\begin{figure} \centering \begin{tikzpicture}[xscale=2]
\node (Label) at  (01.3533,0.7) {\tiny{CD}}; % the label
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](00.6667, 0.5) -- (02.0400, 0.5);
\foreach \x in {00.6667,02.0400} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);

\draw[gray, thick](00.6667, 0) -- (04.0000, 0);
\foreach \x in {00.6667,01.3333,02.0000,02.6667,03.3333,04.0000}\draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
\node (Label) at (00.6667,0.2) {\tiny{1}};
\node (Label) at (01.3333,0.2) {\tiny{2}};
\node (Label) at (02.0000,0.2) {\tiny{3}};
\node (Label) at (02.6667,0.2) {\tiny{4}};
\node (Label) at (03.3333,0.2) {\tiny{5}};
\node (Label) at (04.0000,0.2) {\tiny{6}};
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](01.0367,-00.2500) -- ( 02.2900,-00.2500);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](01.5833,-00.4000) -- ( 02.5300,-00.4000);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](02.1900,-00.6500) -- ( 03.5033,-00.6500);
\node (Point) at (01.0867, 0){};  \node (Label) at (0.5,-00.8500){\scriptsize{OLBoost\_VFDT}}; \draw (Point) |- (Label);
\node (Point) at (01.6333, 0){};  \node (Label) at (0.5,-01.1500){\scriptsize{OLBoost\_SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (02.2400, 0){};  \node (Label) at (0.5,-01.4500){\scriptsize{OLBoost\_SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (03.4533, 0){};  \node (Label) at (4.5,-00.8500){\scriptsize{SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (03.0867, 0){};  \node (Label) at (4.5,-01.1500){\scriptsize{SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (02.4800, 0){};  \node (Label) at (4.5,-01.4500){\scriptsize{VFDT}}; \draw (Point) |- (Label);
\end{tikzpicture}
\caption{Nemenyi test comparing accuracy.}
\label{fig:nemenyi_acc}
\end{figure}


==> old/ESANN_OLBoost_MEM.tex <==
\begin{figure} \centering \begin{tikzpicture}[xscale=2]
\node (Label) at  (01.3533,0.7) {\tiny{CD}}; % the label
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](00.6667, 0.5) -- (02.0400, 0.5);
\foreach \x in {00.6667,02.0400} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);

\draw[gray, thick](00.6667, 0) -- (04.0000, 0);
\foreach \x in {00.6667,01.3333,02.0000,02.6667,03.3333,04.0000}\draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
\node (Label) at (00.6667,0.2) {\tiny{1}};
\node (Label) at (01.3333,0.2) {\tiny{2}};
\node (Label) at (02.0000,0.2) {\tiny{3}};
\node (Label) at (02.6667,0.2) {\tiny{4}};
\node (Label) at (03.3333,0.2) {\tiny{5}};
\node (Label) at (04.0000,0.2) {\tiny{6}};
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](00.6167,-00.2500) -- ( 01.7433,-00.2500);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](01.6433,-00.4000) -- ( 03.0167,-00.4000);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](02.9167,-00.2500) -- ( 04.0500,-00.2500);
\node (Point) at (00.6667, 0){};  \node (Label) at (0.5,-00.8500){\scriptsize{SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (01.6933, 0){};  \node (Label) at (0.5,-01.1500){\scriptsize{OLBoost\_SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (01.6933, 0){};  \node (Label) at (0.5,-01.4500){\scriptsize{SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (04.0000, 0){};  \node (Label) at (4.5,-00.8500){\scriptsize{OLBoost\_VFDT}}; \draw (Point) |- (Label);
\node (Point) at (02.9667, 0){};  \node (Label) at (4.5,-01.1500){\scriptsize{vfdt}}; \draw (Point) |- (Label);
\node (Point) at (02.9667, 0){};  \node (Label) at (4.5,-01.4500){\scriptsize{OLBoost\_SVFDT-II}}; \draw (Point) |- (Label);
\end{tikzpicture}
\caption{Nemenyi test comparing memory consumption.}
\label{fig:nemenyi_mem}
\end{figure}



==> old/ESANN_OLBoost_TIME.tex <==
\begin{figure} \centering \begin{tikzpicture}[xscale=2]
\node (Label) at  (01.3533,0.7) {\tiny{CD}}; % the label
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](00.6667, 0.5) -- (02.0400, 0.5);
\foreach \x in {00.6667,02.0400} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);

\draw[gray, thick](00.6667, 0) -- (04.0000, 0);
\foreach \x in {00.6667,01.3333,02.0000,02.6667,03.3333,04.0000}\draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
\node (Label) at (00.6667,0.2) {\tiny{1}};
\node (Label) at (01.3333,0.2) {\tiny{2}};
\node (Label) at (02.0000,0.2) {\tiny{3}};
\node (Label) at (02.6667,0.2) {\tiny{4}};
\node (Label) at (03.3333,0.2) {\tiny{5}};
\node (Label) at (04.0000,0.2) {\tiny{6}};
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](01.0967,-00.2500) -- ( 01.7433,-00.2500);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](01.6433,-00.4000) -- ( 03.0767,-00.4000);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm}, very thick, color = black](02.9767,-00.2500) -- ( 03.8033,-00.2500);
\node (Point) at (01.1467, 0){};  \node (Label) at (0.5,-00.8500){\scriptsize{VFDT}}; \draw (Point) |- (Label);
\node (Point) at (01.2067, 0){};  \node (Label) at (0.5,-01.1500){\scriptsize{SVFDT-I}}; \draw (Point) |- (Label);
\node (Point) at (01.6933, 0){};  \node (Label) at (0.5,-01.4500){\scriptsize{SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (03.7533, 0){};  \node (Label) at (4.5,-00.8500){\scriptsize{OLBoost\_SVFDT-II}}; \draw (Point) |- (Label);
\node (Point) at (03.1467, 0){};  \node (Label) at (4.5,-01.1500){\scriptsize{OLBoost\_VFDT}}; \draw (Point) |- (Label);
\node (Point) at (03.0267, 0){};  \node (Label) at (4.5,-01.4500){\scriptsize{OLBoost\_SVFDT-I}}; \draw (Point) |- (Label);
\end{tikzpicture}
\caption{Nemenyi test comparing time costs.}
\label{fig:nemenyi_time}
\end{figure}

